ConMatch: Semi-Supervised Learning with Confidence-Guided Consistency Regularization

We present a novel semi-supervised learning framework that intelligently leverages the consistency regularization between the model's predictions from two strongly-augmented views of an image, weighted by a confidence of pseudo-label, dubbed ConMatch. While the latest semi-supervised learning methods use weakly- and strongly-augmented views of an image to define a directional consistency loss, how to define such direction for the consistency regularization between two strongly-augmented views remains unexplored. To account for this, we present novel confidence measures for pseudo-labels from strongly-augmented views by means of weakly-augmented view as an anchor in non-parametric and parametric approaches. Especially, in parametric approach, we present, for the first time, to learn the confidence of pseudo-label within the networks, which is learned with backbone model in an end-to-end manner. In addition, we also present a stage-wise training to boost the convergence of training. When incorporated in existing semi-supervised learners, ConMatch consistently boosts the performance. We conduct experiments to demonstrate the effectiveness of our ConMatch over the latest methods and provide extensive ablation studies. Code has been made publicly available at https://github.com/JiwonCocoder/ConMatch.

==> algorithm/algo.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\begin{scriptsize}

    \PyCode{\rc{for} (x, y), (u\_w, u\_s1, u\_s2) \rc{in} loader:} \\
        \Indp

        \PyCode{(feat\_x, logit\_x), (feat\_u\_w, logit\_u\_w) = model(x), model(u\_w)} \\
        \PyCode{(feat\_u\_s1, logit\_u\_s1), (feat\_u\_s2, logit\_u\_s2) = model(u\_s1), model(u\_s2)} \\

        \PyCode{} \\
        
        \PyComment{confidence estimation} \\
        \PyCode{c\_x = confidence\_estimator(feat\_x, logit\_x)}\\ 
        \PyCode{c\_s1 = confidence\_estimator(feat\_u\_s1, logit\_u\_s1)}\\ 
        \PyCode{c\_s2 = confidence\_estimator(feat\_u\_s1, logit\_u\_s2)}\\ 
        
        \PyCode{} \\

        
        \PyComment{confidence estimator loss} \\
        \PyCode{c\_gt = (torch.argmax(logits\_x, dim=1) == y).float()} \\
        \PyCode{loss\_conf = BCELoss(c\_x, c\_gt)} \\
        \PyCode{loss\_conf += c\_s1 * CrossEntropy(logit\_u\_s1.detach(), logit\_u\_w.detach())} \\
        \PyCode{loss\_conf += c\_s2 * CrossEntropy(logit\_u\_s2.detach(), logit\_u\_w.detach())} \\
        \PyCode{loss\_conf += lam\_reg * (log(1/c\_s1)+log(1/c\_s2)) } \\

        \PyCode{} \\
        
        \PyComment{confidence guided self-supervision loss} \\
        \PyCode{loss\_cgs = c\_s1.detach() * CrossEntropy(logit\_u\_s2, logit\_u\_s1.detach())} \\
        \PyCode{loss\_cgs += c\_s2.detach() * CrossEntropy(logit\_u\_s1, logit\_u\_s2.detach())} \\

        \PyCode{} \\

        \PyComment{semi-supervision loss} \\
        \PyCode{loss\_sup = CrossEntropy(logits\_x, y\_b)} \\
        \PyCode{loss\_un = max\_prob(u\_w).ge(tau).float()} \\
        \Indp \Indp \Indp
        \PyCode{* CrossEntropy(logit\_u\_s1, logit\_u\_w.detach())} \\
        \Indm \Indm \Indm
        \PyCode{loss\_un += max\_prob(u\_w).ge(tau).float()} \\
        \Indp \Indp \Indp
        \PyCode{* CrossEntropy(logit\_u\_s2, logit\_u\_w.detach())} \\
        \Indm \Indm \Indm

        \PyCode{} \\

        \PyCode{loss = loss\_sup + loss\_conf + loss\_cgs + loss\_un} \\
        
        \PyCode{loss.backward()} \\
        
        \PyCode{} \\
        \PyComment{update parameters} \\
        \PyCode{update(model, confidence\_estimator)} \\
        
        
        
        \Indm
        
\end{scriptsize}
\caption{\footnotesize {ConMatch-P (Parametric approach) algorithm}}
\label{algo:algorithm}
\end{algorithm}



==> tables/ablation_similarity.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1}
\caption{
Comparison on error rates for CIFAR-10, CIFAR-100 and SVHN on 5 different folds.  Ours denotes applying non-parametric confidence estimation, and Ours$^\dagger$ is parametric confidence estimation. 
}
\label{table:main_table}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}lccc@{}}
\toprule
 &  \multicolumn{3}{c}{Similarity function}\\
 \cline{2-4}
Method &  L2 distance & Cosine similarity & Cross entropy\\
% &   \multicolumn{3}{c}{\# Labeled samples} & \multicolumn{3}{c}{\# Labeled samples} \\\
\midrule
CGS-NP & & & \\  
CGS-P & & &  \\ 
\bottomrule
\end{tabular}
}
\end{table}



==> tables/baseline_comparison2.tex <==

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\caption{
Comparison between the SSL baseline with our proposed method on CIFAR-10. Numbers are error rates across 3 runs.
}
\label{table:baseline_ablation}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{@{\extracolsep{4pt}}lccccccc@{}}
\toprule
Method  & & & 40 && 250 &&& 
\midrule
(Baseline) FixMatch~\cite{sohn2020fixmatch}         & &  &&&&\\
Ours &  & \\
  \hline \hline
(Baseline) FlexMatch~\cite{zhang2021flexmatch}         & &  \\
Ours    &&& 77.25 $\pm$ 0.52 && 77.25 $\pm$ 0.52 && \\ 
\bottomrule
\end{tabular}
}
\end{table}

% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \caption{
% Comparison between the image-based baseline with our proposed feature-based augmentation method on DomainNet with 1) unlabeled data coming from the same domain as the labeled target ($r_u = 0 \%$), and 2) half of unlabeled data coming from the same domain as the labeled target and the other half from shifted domains ($r_u = 50 \%$).
% Numbers are error rates across 3 runs.
% }
% \label{table:domainnet}
% \resizebox{0.6\textwidth}{!}{
% \begin{tabular}{@{\extracolsep{4pt}}lcc@{}}
% \toprule
% & & 40 & 250 \\
% Method & 40 & 250 \\
% \midrule
% (Baseline) FixMatch         & 56.63 $\pm$ 0.17 & 65.82 $\pm$ 0.07 \\
% Ours  & 40.66 $\pm$ 0.60 & 54.01 $\pm$ 0.66 \\ 
% Ours $^\dagger$ & \multicolumn{2}{c}{77.25 $\pm$ 0.52} \\ \hline \hline
% (Baseline) FlexMatch         & 56.63 $\pm$ 0.17 & 65.82 $\pm$ 0.07 \\
% Ours  & 40.66 $\pm$ 0.60 & 54.01 $\pm$ 0.66 \\ 
% Ours $^\dagger$ & \multicolumn{2}{c}{77.25 $\pm$ 0.52} \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> tables/deprecated_main_table.tex <==



\begin{table}[t]
\caption{\textbf{Quantitative evaluation on CIFAR-10~\cite{krizhevsky2009learning} and SVHN~\cite{netzer2011reading}.} The best results are in bold, and the second best results are underlined. }
\begin{center}
\scalebox{0.95}{
\begin{tabular}{l|ccc|c|cc}
\hlinewd{0.8pt}
\multirow{2}{*}{Methods} & \multicolumn{3}{c|}{CIFAR-10~\cite{krizhevsky2009learning}}  &\multicolumn{1}{c|}{CIFAR-100~\cite{krizhevsky2009learning}}    & \multicolumn{2}{c}{SVHN~\cite{netzer2011reading}}      \\ \cline{2-7} 
                                        & 40             & 250                 & 4000              &400      & 40      & 250
                                        \\ 
\hline
Pseudo-Label~\cite{lee2013pseudo}     & -             & 51.22\tiny{±0.43}    & 83.91\tiny{±0.28} &-        & -       & 79.79\tiny{±1.09}   \\
Pi-Model~\cite{laine2016temporal}     & -            & 45.74\tiny{±3.97}    & 85.99\tiny{±0.38}  &-        & -       & 81.04\tiny{±1.92}   \\
Mean Teacher~\cite{tarvainen2017mean} & -             & 67.68\tiny{±2.30}     & 90.81\tiny{±0.19}  &-        & -       & 96.43\tiny{±0.11}    \\
MixMatch~\cite{berthelot2019mixmatch} & 51.90\tiny{±11.76} & 88.97\tiny{±0.85} & 93.58\tiny{±0.10} & 32.39\tiny{±1.32} & 57.45\tiny{±14.53} & 96.02\tiny{±0.26}  \\
UDA~\cite{xie2020unsupervised}        & 71.95\tiny{±9.64}  & 91.18\tiny{±1.08} & 95.12\tiny{±0.18} & 40.72\tiny{±0.88} & 47.37\tiny{±20.51} & 94.31\tiny{±2.76}   \\
CoMatch~\cite{li2021comatch}    & 91.51\tiny{±2.15}    & -                   & -                   & -       & -       & -               \\
Dash (RA)~\cite{xu2021dash}   & 86.78\tiny{±3.75}  & 95.44\tiny{±0.13}       & 95.92\tiny{±0.06}  & 55.24\tiny{±0.96}    & -          & -       \\ 
FixMatch (RA)~\cite{sohn2020fixmatch} & 86.19\tiny{±3.37}  & 94.93\tiny{±0.65} & 95.74\tiny{±0.05} & 51.15\tiny{±1.75} & 96.04\tiny{±2.17} & 97.52\tiny{±0.38}  \\ 
FlexMatch~\cite{zhang2021flexmatch} & 95.03\tiny{±0.06}  & 95.02\tiny{±0.09} & 95.81\tiny{±0.01} & 60.06\tiny{±1.62} & 91.81\tiny{±3.20}                   & -   \\ \hline
\textbf{Ours}                       & -                   & -                & -                & -                 & -               & -    \\
\textbf{Ours*}                      & -                   &  -               & -                & -                 & -               & -    \\ \hlinewd{0.8pt}

\end{tabular}}
\end{center}

\label{quan_table_cifar10_SVHN}
\end{table}
